Dynamic Sampling Rate: Harnessing Frame Coherence in Graphics Applications for Energy-Efficient GPUs

In real-time rendering, a 3D scene is modelled with meshes of triangles that the GPU projects to the screen. They are discretized by sampling each triangle at regular space intervals to generate fragments which are then added texture and lighting effects by a shader program. Realistic scenes require detailed geometric models, complex shaders, high-resolution displays and high screen refreshing rates, which all come at a great compute time and energy cost. This cost is often dominated by the fragment shader, which runs for each sampled fragment. Conventional GPUs sample the triangles once per pixel, however, there are many screen regions containing low variation that produce identical fragments and could be sampled at lower than pixel-rate with no loss in quality. Additionally, as temporal frame coherence makes consecutive frames very similar, such variations are usually maintained from frame to frame. This work proposes Dynamic Sampling Rate (DSR), a novel hardware mechanism to reduce redundancy and improve the energy efficiency in graphics applications. DSR analyzes the spatial frequencies of the scene once it has been rendered. Then, it leverages the temporal coherence in consecutive frames to decide, for each region of the screen, the lowest sampling rate to employ in the next frame that maintains image quality. We evaluate the performance of a state-of-the-art mobile GPU architecture extended with DSR for a wide variety of applications. Experimental results show that DSR is able to remove most of the redundancy inherent in the color computations at fragment granularity, which brings average speedups of 1.68x and energy savings of 40%.

==> Results/tmppunt2.tex <==
%%original
The activity reduction experiences very minor variation across frames. Because consecutive frames tend to be very similar, the ASR and its resultant savings remain somewhat constant over time. On the other hand, individual tiles may require different sampling rates over time. DSR is able to capture those changes and adjust the sampling rate accordingly. Figure \ref{fig:srtiles} illustrates this by depicting the sampling rate of 4 tiles over several frames, starting at the beginning of the execution of the application. We can observe that DSR starts sampling all the tiles at the maximum rate, 1x (\circled{1}).

%frase original lleugerament variada

Because consecutive frames tend to be very similar, the ASR of an application and its resultant savings remain somewhat constant over time. However, individual tiles may require different sampling rates as the scene experiences minor variations every frame. DSR is able to capture those changes and adjust the sampling rate accordingly. Figure \ref{fig:srtiles} illustrates ...

%més canvis, ara posant el focus als canvis enlloc que la mitjana es manté

Even though consecutive frames tend to be very similar, the minor variations that a scene may experience over time could change the sampling rate requirements of individual tiles. DSR is able to capture those changes and adjust the sampling rate accordingly. Figure \ref{fig:srtiles} illustrates ...


%%deixar de banda completament la frase que la mitjana es manté

DSR is able to capture changes that occur over time in a scene and adjust the sampling rate of individual tiles accordingly.  Figure \ref{fig:srtiles} illustrates ...



